On Bridging the Gap between Mean Field and Finite Width in Deep Random Neural Networks with Batch Normalization

Mean field theory is widely used in the theoretical studies of neural networks. In this paper, we analyze the role of depth in the concentration of mean-field predictions, specifically for deep multilayer perceptron (MLP) with batch normalization (BN) at initialization. By scaling the network width to infinity, it is postulated that the mean-field predictions suffer from layer-wise errors that amplify with depth. We demonstrate that BN stabilizes the distribution of representations that avoids the error propagation of mean-field predictions. This stabilization, which is characterized by a geometric mixing property, allows us to establish concentration bounds for mean field predictions in infinitely-deep neural networks with a finite width.

==> arXiv_backup/assumption.tex <==


\section{Bounding singularity at infinite depth}
In this section, we will examine the deviations of parameters from mean field predictions in the fixed point grand matrix. We will divide this analysis into two main parts: the first part will focus on understanding the dynamics of the mean field recurrent step, and the second part will focus on understanding the dynamics of finite width systems in comparison to mean field or infinite width systems.


Before moving on to the first theorem, it is important to note that the BN operator centering causes the smallest eigenvalue to be zero in the direction of $\1_n.$ Therefore, we will consider the G-matrices after projection onto this $n-1$-dimensional hyperplane. Let where $B=\R^{n\times (n-1)}$ be an orthonormal matrix, such that its columns spans the space $\{x\in\R^n: \ip{\1_n}{x}=0\}.$ Therefore, we will track the dynamics of centered-Gram matrices $\overline{G}_\ell=B^\top G_\ell B.$  We will track regularity of G-matrices $\gamma(\overline G_\ell),$ aiming to show that they can be probability of the event $\gamma(G_\ell)=0$ is zero, regardless of $\ell$. 

In particular, we will be interested the geometric series $g_\ell:=\gamma(G_{\ell+1})/\gamma(G_\ell).$ If we can show that the product $\prod_{\ell}^\infty g_\ell > 0,$ with positive probability, then starting from $\gamma(G_0)>0$ we must have $\gamma(G_{\ell})>0$ with some positive probability for $\ell=\infty.$ Equivalently, we can show that sum of their logarithms is lower bounded: $\sum_{\ell=0}^\infty \log(g_\ell)> -\infty.$

\subsection{Contraction in mean field $d=\infty$}
We aim to demonstrate that in the mean-field step~\eqref{eq:MF_recurrence}, the conditioning of G-matrix improves. 
In one particular case, when using a linear activation function, we are able to directly show that this step leads to an improvement in the conditioning of the gram matrix. However, this is complicated to prove directly due to dependencies introduced by the batch normalization operator, which involves taking multiple samples within a batch, making it difficult to take expectations and simplify the calculations. Although we cannot rigorously prove this improvement in conditioning, by a mean field approximation, we can show that most common types of activations satisfy this property. 


\begin{lemma}
\label{lem:expectation_ratio}
Let $\rvx\sim\Normal(0,C)$ be an $n$-dimensional Gaussian with trace-normalized covariance, and define $C'=\E_{w\sim\Normal(C)}(\BN(w))^{\otimes 2}.$ We have 
 We have
\begin{align}
\gamma\left(C'\right) \ge \gamma(C)\left(1+\frac{2}{n+1}(1-\gamma(C)) \right)
\end{align}
\end{lemma}

\subsection{Contraction in Finite Field $d<\infty$}
To begin, we will examine the probability that the norms of each row or any row of the matrix may revert back to zero, as well as the probability that the minimum eigenvalues of these matrices may become zero. This is important to consider, as if there is any strictly positive probability of such an event occurring in the infinite depth regime, it is guaranteed to happen.

To control these deviations, we will rely on powerful results from free probability theory about Wishart matrix distributions. However, to do this, we will have to rely on several mean field approximations. The mean field approximation implies that we approximate distributions as Gaussian distributions with similar first and second moments when we have a sufficient number of observations.

To accomplish this, we will compute the first and second moments and replace a distribution with an equivalent moment, using well-known facts about Gaussian distributions. Additionally, we will assume certain structures or properties about the activation function that would ensure that the values of the activations will not converge to zero if the values of x are not nearly zero. This is important as it allows us to bound the probability of negative moments, which are crucial for balancing the minimum eigenvalues.




==> arXiv_backup/intro.tex <==
\section{Introduction}
\subsection{Depth is essential but slow to train} 
Deep neural networks have achieved
state-of-the-art performance in numerous tasks \cite{lecun2015deep, he2016deep, klambauer2017self, radford2019language}. While even a 2-layer MLP is a universal approximator~\cite{}, deeper networks become exponentially more expressive~\cite{poole2016exponential}, achieving strong generalization performance. Training deep models is slow due to
vanishing/exploding gradients and slow signal propagation
in depth~\cite{he2015delving}. 
% \subsection{Practical remedies for training deep networks}
Numerous approaches have been proposed to accelerate optimization of deep neural networks, including residual connections~\cite{he2016deep}, careful scaling of the weights~\cite{glorot2010understanding,xiao2018dynamical}, and batch normalization~\cite{ioffe2015batch} to remove co-variate shift. 

\subsection{Spectrum of representations is key}
In a theoretical study\cite{pennington2017nonlinear}
demonstrated that dynamical isometry~\cite{saxe2013exact} is a key indicator of fast training, and tight spectral concentration of Jacobian can speed up training by orders of magnitude~\cite{pennington2018emergence}.
In separate theoretical works~\cite{}, it is shown that in a random Multi-Layer Perceptron (MLP), batch normalization prevents stable-rank of representations from collapsing~\cite{}, and makes them orthogonal in depth\cite{}, and the empirical results connect the speedup in training with the spectral characteristics of representations at initialization~\cite{}. In light of these findings, it is important to have a theoretical understanding of how the spectra depends on the normalization layers, and choice of activation function. In the current work, we give a non-asymptotic characterization of the entire spectra of representations of a MLP at initialization with batch normalization. 

% \subsection{Informal results}
\paragraph{Our main contributions}
The key step in our analysis is that second-moments of representations approaches approach limiting matrix $C_*$ with depth, which is derived in close-form. This analysis shows surprising consequences of choice of activation on the limiting spectra of representations.
The spectral characterization analysis extends the existing results on MLP with random weights in several important ways:
\begin{itemize}
    \item The spectral characterization strengthens the orthogonality of representations result proven 
    \item We extend the result from MLP with linear activation to MLP with a wide range of non-linear activations.
    \item The subsequent Gaussian-approximation result extends the existing bounds to the finite width and depth regime.
\end{itemize}

==> arXiv_backup/introduction_new.tex <==
\section{Introduction}

Deep neural networks have achieved state-of-the-art performance in many machine learning tasks, including image recognition~\cite{lecun2015deep}, natural language processing~\cite{radford2019language}, and speech recognition~\cite{he2016deep}. These models are able to achieve strong generalization performance due to their high capacity, which increases exponentially with the number of layers~\cite{poole2016exponential}. However, training deep models becomes increasingly slow as the number of layers increases~\cite{he2015delving,he2016deep}.

To understand the reasons for this training slowdown, researchers have examined the role of depth at initialization~\cite{pennington2017nonlinear,kohler2019exponential,daneshmand2020batch,daneshmand2021batch}. Standard initialization schemes often lead to a systematic issue where the outputs of deep networks become aligned along the same direction, regardless of the inputs~\cite{daneshmand2020batch}. This issue, known as rank collapse, occurs in various neural architectures, including MLPs~\cite{saxe2013exact}, convolutional networks~\cite{daneshmand2020batch}, and transformers~\cite{anagnostidissignal}. Rank collapse leads to ill-conditioning of the input-output Jacobian, which slows training~\cite{pennington2018emergence}. Saxe et al.\cite{saxe2013exact} showed that avoiding rank collapse can accelerate the training of deep linear networks, and this concept has been the focus of numerous theoretical and experimental studies\cite{pennington2018emergence,daneshmand2020batch,daneshmand2021batch}.

One way to avoid rank collapse is through the use of batch normalization (BN)\cite{ioffe2015batch}. BN has been shown to significantly enhance the training of neural networks\cite{ioffe2015batch}. Recent studies have linked the effectiveness of BN to the spectral characteristics of representations at initialization~\cite{kohler2019exponential,daneshmand2020batch,daneshmand2021batch}. BN has been shown to avoid rank collapse in linear neural networks by iteratively orthogonalizing the representations across layers~\cite{daneshmand2021batch}. However, these results only hold for linear activations~\cite{daneshmand2020batch,daneshmand2021batch}. 

Building on previous work on linear random deep neural networks with BN, we characterize the influence of the activation function on the spectra of representations in depth. Our main contribution is a non-asymptotic characterization of the entire spectra of representations of a MLP at initialization with batch normalization. To our surprise, we show that it is possible to approximate the spectra of random representations in deep layers of neural networks with BN, despite the randomness of weights.

Our results are novel in several ways:

\begin{itemize}
    \item We prove that BN can avoid the rank collapse issue in networks with ReLU and a wide range of odd activations. This conjecture was previously proposed in~\cite{daneshmand2020batch}.
    \item Our analysis can approximate the spectra of representations for a broad family of non-linear activations beyond ReLU and odd activations.
    \item  We establish a novel method to predict the stationary distribution of a family of contracting Markov chains.
\end{itemize}

% \section{Introduction}

% % \subsection{Depth is essential} 
% Deep neural networks have achieved
% state-of-the-art performance in numerous machine learning tasks \cite{lecun2015deep, he2016deep, klambauer2017self, radford2019language}. Deeper models are exponentially more expressive ~\cite{poole2016exponential}, and achieve strong generalization performance~\cite{gissin2019implicit}. 
% % \subsection{Practical remedies for training deep networks}
% Despite advantages of depth, training deep models becomes slow as the networks grow in depth~\cite{he2015delving,he2016deep}. 
% % , which was missing from the practical approaches~\cite{glorot2010understanding,xiao2018dynamical,he2016deep}. 
% % \subsection{Practical remedies for training deep networks}
% % Numerous approaches have been proposed to accelerate optimization of deep neural networks~\cite{glorot2010understanding,xiao2018dynamical,he2016deep}.  


% % \subsection{Spectrum of representations is key for fast training}

% To explain the training slowdown with depth, a line of research investigate the role of depth at initialization~\cite{pennington2017nonlinear,kohler2019exponential,daneshmand2020batch,daneshmand2021batch}.
% Standard initialization schemes suffer from a systematic issue: When the networks grow in depth, the outputs become align along the same direction independent from the inputs~\cite{daneshmand2020batch}. In other words, the rank of the output matrix for a batch of data collapses to one. 
%  This issue arises in various neural architectures, including MLPs\cite{saxe2013exact}, Convolution nets\cite{daneshmand2020batch}, and transformers\cite{anagnostidissignal}.  This collapse causes ill-conditioning of input-output Jacobean that dramatically slows training~\cite{pennington2018emergence}. \cite{saxe2013exact} shows avoiding the rank collapse of outputs accelerates training of deep linear networks. Since then, tackling ill-conditioned outputs has become the focus of various theoretical and experimental studies\cite{pennington2018emergence,daneshmand2020batch,daneshmand2021batch}.


% % \subsection{Batch Normalization helps training by preserving spectra}
% Batch Normalization (BN) significantly enhances training of neural networks\cite{ioffe2015batch}.
% Recent studies link the speedup in training with batch normalization to the spectral characteristics of representations at initialization~\cite{kohler2019exponential,daneshmand2020batch,daneshmand2021batch}.
% While conventional neural nets are prune to the rank collapse ~\cite{daneshmand2020batch}, batch normalization avoids the rank collapse~\cite{daneshmand2020batch}. This statement is proven for linear neural networks showing that batch normalization iteratively orthogonalize representation across the layers\cite{daneshmand2021batch}. 
% Nevertheless, these theoretical result only hold for linear activations~\cite{daneshmand2020batch,daneshmand2021batch}.


% % \subsection{Informal results}
% % \subsection{Our main contributions}

% Building upon studies of linear random deep neural nets with BN, we  characterize the influence of activation function on spectra of representations in depth.
% Our main contribution of this is a non-asymptotic characterization of the entire spectra of representations of a MLP at initialization with batch normalization. Surprisingly, we show one can approximate the spectra of random representation in deep layers of neural nets with batch normalization, despite the randomness of weights.
% Our results are novel from various aspects:
% % The spectral characterization analysis extends the existing results on MLP with random weights in several important ways:
% \begin{itemize}
%     \item We prove avoiding the rank collapse issue by batch normalization for networks with ReLU and wide range of odd activations. This conjecture is proposed by \cite{daneshmand2020batch}. 
%     \item Our can approximate the spectra of representation for  a broad family of non-linear activation beyond ReLU and odd activations.
%     \item We establish a novel method to predict the stationary distribution of a family of contracting Markov chains. 
%     % \item Our analysis derives the first non-asymptotic Gaussian-approximation for outputs of random neural networks with  finite width. \textcolor{blue}{Hadi: does not match our story. We can just mention this later and not in the intro.}
% \end{itemize}

==> arXiv_backup/moment_stability_argument.tex <==
\section{Viewing stability via stabilitiy of moments}
Understanding the hidden representations of a multi-layer perceptron (MLP) is challenging due to the random rotation of feature space induced by random matrix products \textcolor{blue}{You mean non-linear transformation of random variables. The product is only for linear neural nets.}. Many deterministic patterns that emerge at depth, such as vanishing or exploding norms, are hallmarks of undesirable network initialization. Therefore, we propose to focus on the probability distribution function \textcolor{blue}{Is this really what we propose? We just need the geometrically contraction. Justifying that assumption is much more important to explain how we prove the main theorem} of the representations, as it is a deterministic function, and model these hidden representations as a Markov chain \textcolor{blue}{What do you mean by modeling representations as Markov chain by distributions? The chain of representations is a Markov chain. }. We aim to uncover the stable distribution of this chain \textcolor{blue}{ Why do you want to uncover it? You can say that when the chain is contracting it converges to the stationary distribution, so we analyze its stationary distribution}, which provides a measure of stochastic stability \textcolor{blue}{a measure of statistic stability?}. The remainder of this section is dedicated to studying the structures that emerge as a result of this stability and showing that they remain remarkably accurate in finite parameter regimes. \textcolor{blue}{Stationary distribution or stable distribution? Do not use two different words for the same thing. Stationary is formal statement. }

\paragraph{Stable Moment Relaxation of Markov Chains}
Deriving a closed-form solution for the stationary distribution of a neural network \textcolor{blue}{Stationary distribution of neural net? What do you mean by that?} is highly non-trivial \textcolor{blue}{why?}. One way to overcome this technical difficulty is to study the moments under the infinite-width limit \textcolor{blue}{It not convincing to me at all. Why it does help?}, which leads to mean field theory. Conditioned on the previous layer, moments of representations are deterministic, and can serve as a proxy for the stable distribution. Therefore, we introduce the moment-analogue of a stable distribution:
\begin{align}\label{eq:stable_moment_dist}
\E_{\T_\#\mu}[X^{k\otimes}] = \E_{\mu}[X^{k\otimes}]
\end{align}
\textcolor{blue}{Do we use stable moments using $T$? The stable moments are not obtained by a Markov chain in the same state with the same transition map. This is a wrong statement.}
This definition shows that this is a much weaker stability than the stationary distribution. As the distribution shifts from $\mu$ to $\T_\#\mu$, it does not necessarily transfer to next steps. In other words, while $\T_\#\mu$ has similar moments to $\mu$, moments of $\T^k_\#\mu$ might quickly diverge from this value. This means that the deviations in the chain updates will propagate or even amplify through successive chain updates $\T$ \textcolor{blue}{One can argue if we have the contracting this won't happens. We are not tracking the moment of the Markov chain Amir, we are tracking another difference equation which is difficult to relate to the current finite dimenional Markov chain. }.

If the dynamics of moments exhibit enough stability, we can expect that the stable distributions are close to the stationary distribution $\mu_\infty$. If we can show that any distribution $\hat\mu$ with stable $k$-th moment is close to the moments of the stationary distribution $\mu_\infty$, then we can expect the moments of the two to be close $\E_{\hat\mu}[x^{k\otimes}] \approx \E_{\mu_\infty}[x^{k\otimes}]$ \textcolor{blue}{Why? Prove it.}. Therefore, analyzing the stationary distribution can be reduced to the much simpler problem of finding a candidate $\hat\mu$ that passes the stable moment certificate in~\eqref{eq:stable_moment_dist}, without sacrificing too much accuracy. \textcolor{blue}{This not true and can be stated in the proof sketch. Why person cares about this results? If you want to lead the person through you need to give examples and lemma with proofs. This is not convincing at all.  }


Rather than computing or bounding these moments directly, if we can prove that the distribution of $\T(x)$ is highly concentrated, it suffices to only study first and second moments. This leads to Chernoff-type bounds, by only controlling the second moments. However, this requires delving into the inner machinery of the MLP chain, instead of the black-box approach we have taken thus far. As we will show later in this section, the MLP chain with normalization demonstrates a remarkable stability and high concentration needed \textcolor{blue}{This should be a remark after the main theorem.We did not control the moments first right? We first derive a condidate for the stationary distribution. Then, the got the 
concentration result. Please make sure all statements have to be correct. Each word and each sentence. Add words if they lead readers to the main result. Do not talk about the proof techniques before even saying what is the result.}. 

Before stating our results, let us first discuss the issue of propagating errors at depth as an analysis problem.

==> arXiv_backup/preliminaries.tex <==



% \section{How Can Errors Propagate Through Depth?}
 

% \textit{Deep mean field}
% In order to understand the discrepancy between shallow and deep mean field analysis, i.e., infinite-width-and-depth regime, we need to carefully analyze the trace and determinant of the gram matrix as we consider depth and width asymptotically.

% The trace of the gram matrix, $\E \tr(C_\ell)$, can be calculated using the circular property of trace. This equals $X^\top \tr X^\top X\E (\prod_k^\ell W_k^\top W_k)$. Since the matrices $W_k$ are independent, we can take the expectation inside, which is $\tr X^\top X\prod_k^\ell (\E W_k^\top W_k)$. By construction of the matrices $W_k$, we have $\E W_k^\top W_k = I_n$, implying $\E \tr(C_\ell) = \tr X^\top X = n$. This term is consistent with the shallow analysis. Furthermore, from the fact that trace is the sum of eigenvalues we can conclude $\E \lambda_1(C_\ell)\ge \frac1n \tr(I_n) = 1.$

% The determinant of the gram matrix, $\E \det(C_\ell)$, can be calculated using properties of determinant and results for determinant of Wishart matrices. We can show that $\E \det(C_\ell)\lesssim \exp(-\nfrac{\ell n^2}{2d})$. Considering the fact that $\lambda_n(C_\ell)\le \det(C_\ell)^{\nfrac1n}$, we have $\E \lambda_n(C_\ell)\le \exp(-\nfrac{ n \ell}{2d})$.
% Combining these results, we can deduce the deep mean field prediction for the conditioning of the gram matrix: $\E[\kappa(C_\ell)] \gtrsim \exp(\frac{n \ell}{2d})$. 


% Moreover, the formula $\exp(-n r)$ which is significantly deviates from the shallow mean field when $\nfrac{\ell}{d}=r$ is kept as a constant when $d\to\infty$. This formula hints at an interesting interplay between depth, batch size, and width that acts as an indicator of the discrepancy between shallow and deep mean field analysis, which can be summarised as: \begin{align}\label{eq:mean_field_discrepancy_informal}
% \text{shallow/deep conditioning} \approx \exp(\frac{\text{batch}\cdot \text{depth}}{\text{width}})
% \end{align}

% This is largely consistent with an elegant observation by~\cite{li2022neural}, showing that the error of an infinite-width-and-depth network behaves like a geometric Brownian motion, with depth playing the role of time. By approximating the dynamics of Gram matrices with an SDE, they accurately predict the degenerate outputs for vanilla MLP in realistic settings. 

% It's important to note the discrepancy is not universal for all activation functions. In fact, ~\cite{li2022neural} leverage their SDE approximation to carefully shape activation functions to arrive at non-degenerate Gram matrices in infinite-depth. However, this does not address the stabilizing effects of normalization in the absence of activation shaping, which is the main focus of the current work. 


==> sections/related.tex <==
\section{Related works}

In a seminal work, \citet{neal2012bayesian} established established the elegant connection between infinitely-wide single-layer neural networks and Gaussian processes, thereby connecting parametric learning and non-parametric learning. Since then, the infinite-width regime which underlies mean field theory has been become an important tools to analyze neural networks.


\textit{Initialization.} Mean field analysis has been used to develop enhanced initialization for deep neural networks~\cite{pennington2018emergence,pennington2017nonlinear}. 
\citet{xiao2018dynamical} use mean field analysis to develop an initialization that allows the training of convolutional layers with 10000 layers.



\textit{Optimization.} \cite{bach2021gradient} establishes the elegant link between gradient descent and Wasserstein gradient flows in the mean field regime, thereby proves the global convergence of gradient descent. The neural tangent kernel has also provided insight into the underlying mechanisms of gradient descent~\cite{jacot2018neural}.



\textit{Generalization.} \citet{chizat2020implicit} prove that gradient descent converges towards maximum margin solutions for neural networks with an infinite number of neurons, demonstrating the implicit bias of training algorithms.


\textit{Architectural components.} Insights from mean field analyses shed light on the essence of batch normalization in deep learning \cite{yang2019mean}. Beyond theoretical insights, mean field analysis has been effectively used in the design of neural architectures~\cite{klambauer2017self}. 
% \end{itemize}

Wide applications of mean field theory has motivated recent research into the gap between mean field theory and the standard non-field regimes. \citet{lewkowycz2020large} argue that optimization with large step-sizes exhibits different dynamics in finite and infinite width regimes. \citet{lee2020finite} show empirically that the difference between optimization for finite-width and infinite-width neural networks. Inspired by these studies, we investigate the role of depth in predictions derived from mean field analyses. Specifically, we focus on the dynamics of representation across the layers of deep random neural networks.

 A recent line of research notes the limitations of mean field theory for deep neural networks, arguing that mean field approximation error accumulates with increasing depth~\cite{seleznova2022neural,li2022neural,matthews2018gaussian}. Indeed, the depth is often considered as curse for mean field theory. The majority of current literature relies on scaling the network width with depth to control the cascade of mean field approximation error \cite{hu2021random,matthews2018gaussian}. Recently, \cite{li2022neural} proposes a novel approach by injecting noise in mean field dynamic, modeling cascade of error across the layers in deep neural networks. Leveraging tools from stochastic differential equations and by shaping activations, \cite{li2022neural} significantly enhances mean field models for conventional neural networks. Here, we demonstrate a neglected facet of error propagation through the depth.
